Targeting Completeness: Using Closed Forms for Size Bounds of Integer Programs

We present a new procedure to infer size bounds for integer programs automatically. Size bounds are important for the deduction of bounds on the runtime complexity or in general, for the resource analysis of programs. We show that our technique is complete (i.e., it always computes finite size bounds) for a subclass of loops, possibly with non-linear arithmetic. Moreover, we present a novel approach to combine and integrate this complete technique into an incomplete approach to infer size and runtime bounds of general integer programs. We prove completeness of our integration for an important subclass of integer programs. We implemented our new algorithm in the automated complexity analysis tool KoAT to evaluate its power, in particular on programs with non-linear arithmetic.

==> evaluation.tex <==
\section{Evaluation and Implementation}
\label{sect:evaluation}
We implemented a prototype of our procedure in our re-implementation of the tool \KoAT, written in \tool{OCaml}.
%
It integrates the computation of size bounds via closed forms for twn-loops and homogeneous (and thus linear) solvable loops into the complexity analysis for general integer programs.\footnote{For a homogeneous solvable loop, the closed form of the twn-loop over $\AA$ that results from its transformation is particularly easy to compute.}
%
In this section, we discuss the strengths of \KoAT{} in an empirical evaluation.
\comment{NL I have added some introductary text.}

To infer local runtime bounds as in \Cref{def:locUpperTimeBound},\oldcomment{JG I removed the related work part here, because it only covered some of the related work, whereas the rest was covered in the introduction.
	%
	Instead of having two parts on related work in different sections, I think it is better to have it all in one place.
	%
	So now all the related work is handled in the introduction.
	%
	I shortened the description of some of the papers on complete results, because otherwise the reader might ask why we describe some results in more detail but not the results of other papers that are cited there as well.
	%
	But I added a sentence in the introduction to compare our complete technique for
        size bounds with the one of \cite{ben-amram2019TightWorstCaseBounds,ben-amram2008LinearPolynomialExponential}.}\oldcomment{For example, for two consecutive loops, the runtime of the second loop depends on the size of the variables after executing the first loop.
	%
	So if we have computed a \emph{local} runtime bound for the second \emph{isolated} loop and want to obtain a \emph{global} runtime bound for the complete program, then we need to consider the size of the variables before evaluating the second loop.
	%
	We incorporate our novel approach to compute size bounds into the setting of general integer programs, i.e.,
	%
	we combine complexity analysis on a Turing-complete language and an approach to compute size bounds for \emph{isolated} loops in a \emph{modular} way.
	%
	We implemented our new approach in the complexity analysis tool \KoAT{}.}
%
\KoAT{}
first applies multiphase-linear ranking functions (see \cite{Festschrift,ben-amram2017MultiphaseLinearRankingFunctions}), which can be done very efficiently.
%
For twn-\linebreak
loops where no finite bound was found, it then uses the computability of runtime bounds for terminating\oldcomment{JG I a added ``terminating'' here, ok?
	%
	You had also written ``and use automorphisms to transform loops into twn form'', but I wasn't sure for which loops you use such automorphisms when computing runtime bounds.
	%
	Only linear ones, only solvable ones, only ones with real eigenvalues?
	%
	Later, you write that runtime bound inference should be extended to prs loops, so it seems that some other class of loops is currently transformed to twn-loops for runtime analysis.}
twn-loops %and use automorphisms to transform loops into twn form
(see \cite{frohn2020TerminationPolynomialLoops,hark2020PolynomialLoopsTermination,lommen2022AutomaticComplexityAnalysis}).
%
When computing size bounds, \KoAT{}
first applies the technique of \cite{brockschmidt2016AnalyzingRuntimeSize} for reasons of efficiency and in case of exponential or infinite size bounds, it tries to compute size bounds via closed forms\linebreak
as in the current paper.
%
Here, \tool{SymPy} \cite{sympy} is used to compute Jordan normal forms for the transformation to twn-loops.
%
Moreover, \KoAT{} applies a local control-flow refinement technique \cite{Festschrift} (using the tool \tool{iRankFinder} \cite{domenech2018IRankFinder}) and preprocesses the program in the beginning, e.g., by extending the guards of transitions with invariants inferred by \tool{Apron}
\cite{jeannet2009ApronLibraryNumerical}.
%
For all SMT problems, \KoAT{} uses \tool{Z3} \cite{moura2008}.
%

To evaluate our new technique, we tested \tool{KoAT} on the 504 benchmarks for \emph{Complexity of} \tool{C} \emph{Integer Programs}
(\tool{CINT})
from the \emph{Termination Problems Data Base} \cite{tpdb} which is used in the annual \emph{Termination and Complexity Competition (TermComp)} \cite{giesl2019TerminationComplexityCompetition}.
%
Here, all variables are interpreted as integers over $\ZZ$ (i.e., without overflows).
%%
To distinguish the original version of \KoAT{} \cite{brockschmidt2016AnalyzingRuntimeSize}
from our re-implementation, we refer to them as \tool{KoAT1} resp.\ \tool{KoAT2}.
%
We used the following configurations of \tool{KoAT2}, which apply different techniques to infer size bounds.

\medskip
\hspace*{-.75cm}
\begin{minipage}{12.5cm}
	\begin{itemize}
		\item[$\bullet\!$] \tool{KoAT2orig} uses the original technique from \cite{brockschmidt2016AnalyzingRuntimeSize} to infer size bounds.
		\item[$\bullet\!$] \tool{KoAT2\,\!+\,\!SIZE} additionally uses our novel approach with \cref{thm:size_bounds_closed_form}, \ref{thm:lift_size_bounds}, and \ref{thm:cycles}.
	\end{itemize}
\end{minipage}

\medskip

%

The \tool{CINT}
collection contains almost only\oldcomment{JG Only 27 of the 504 example are non-linear.
	%
	Approximately 10 of the 15 new examples are non-linear.}
examples with linear arithmetic and the existing tools can already solve most\oldcomment{JG Maybe give the number of examples in the current collection where iRankFinder proves non-termination.
%
It proved non-termination for 118 examples before we added 20 examples in the IJCAR paper.
%
2 of these 20 examples are non-terminating.
%
It should be checked whether iRankFinder can prove their non-termination.
%
All 15 new examples from the current paper are terminating.
NL
The tool \tool{iRankFinder} \cite{domenech2018IRankFinder} proves non-termination for 119 of 519 programs in \tool{CINT${}^+$}.
So, it can prove non-termination for 1 one of the IJCAR examples.\\
JG Thanks, I mentioned that now.
}
of its benchmarks which are not known to be non-terminating.\footnote{\tool{iRankFinder} \cite{domenech2018IRankFinder} proves non-termination for 119  programs  in \tool{CINT}. \tool{KoAT2orig}
already\linebreak infers finite runtimes for 343 of the remaining $504-119 = 386$ examples in
\tool{CINT}.}
%
While most complexity analyzers are essentially restricted to programs with linear arithmetic, our new approach also succeeds on programs with \emph{non-linear} arithmetic.
%
Some programs with non-linear arithmetic could already be handled by
\KoAT{} due to our
integration of the complete technique for the inference of local runtime bounds in
\cite{lommen2022AutomaticComplexityAnalysis}.
%
But the approach from the current paper increases \KoAT's \pagebreak[2] power substantially for programs
(possibly with non-linear arithmetic) where the values of variables computed in
``earlier'' loops influence the runtime of ``later'' loops (e.g., the modification of our
example from \Cref{fig:ITS_solvable_loop} where $t_4$ decreases $x_4$ instead of $x_1$,
see the end of \Cref{ex:global_runtime_bound}).

Therefore, we extended \tool{CINT} by 15 new typical benchmarks including the
programs in \eqref{WhileExample},
\cref{fig:ITS_solvable_loop},
and the modification of \cref{fig:ITS_solvable_loop} discussed above,
as well as several benchmarks from the literature (e.g., \cite{ben-amram2019TightWorstCaseBounds,ben-amram2008LinearPolynomialExponential}), resulting in the collection \tool{CINT${}^+$}.
%
For \tool{KoAT2} and \tool{KoAT1}, we used \tool{Clang} \cite{clang} and \tool{llvm2kittel} \cite{falke2011TerminationAnalysisPrograms} to transform \tool{C} into integer programs as in \Cref{sect:integer_programs}.
%
We compare \tool{KoAT2} with \tool{KoAT1} \cite{brockschmidt2016AnalyzingRuntimeSize} and the tools \tool{CoFloCo} \cite{cofloco2},
%
\tool{MaxCore} \cite{albert2019ResourceAnalysisDriven} with \tool{CoFloCo} in the backend, and \tool{Loopus} \cite{sinn2017ComplexityResourceBound}.
%
These tools also rely on variants of size bounds: \tool{CoFloCo} uses a set of constraints to measure the size of variables w.r.t. their initial and final values, \tool{MaxCore}'s size bound computations build upon \cite{DBLP:conf/popl/CousotH78}, and \tool{Loopus} considers suitable bounding invariants to infer size bounds.\oldcomment{\label{other tools size bounds}
NL Maybe we should add a sentence how these tools use size bounds here: \tool{CoFloCo}: Antonio Flores-Montoya writes ``[..] the used constraint set is a transitive invariant $\varphi$ that relates the initial and final values'' in his diss.
%
\tool{MaxCore} cites \cite{DBLP:conf/popl/CousotH78} for their size bound computations.
%
\tool{Loopus} ``We now contrast our variable bound analysis (function V B ) with classical invariant analysis.''}

\begin{table}[t]
	\makebox[\textwidth][c]{
	  \begin{tabular}{l|c|cc|cc|cc|cc|cc|
              %c|
              c|c}
			                                 & $\landau(1)$ &
                  \multicolumn{2}{c|}{$\landau(n)$} & \multicolumn{2}{c|}{$\landau(n^2)$}
                  & \multicolumn{2}{c|}{$\landau(n^{>2})$} &
                  \multicolumn{2}{c|}{$\landau(\mathit{EXP})$} &
                  \multicolumn{2}{c|}{$< \omega$} & % SR (\%) &
                  $\mathrm{AVG^+(s)}$ & $\mathrm{AVG(s)}$                               \\
			\hline \tool{KoAT2\,\!+\,\!SIZE} & 26           & 233
                        & (2)                                & 71
                        & (1)                                          & 25
                        & (9)                 & 3                 & (2) & 358 & (14) %&
                        %93.25
                        & 9.97 % = (9.00 * 344 + 33.87 * 14)/(344+14)
												& 22.88 % = (22.61 * 504 + 31.98 * 15)/(504+15)
												\\
			\hline \tool{KoAT2orig}          & 26           & 232
                        & (1)                                 & 70
                        &                                              & 15
                        &                     & 5                 & (4) & 348 & (5) %&
                        %90.5
                        & 8.29 % = (8.23 * 343 + 12.68 * 5)/(343+5)
												& 21.52 % = (21.22 * 504 + 31.52 * 15)/(504+15)
												\\
			\hline \tool{MaxCore}            & 23           & 220
                        & (4)                                 & 67
                        & (1)                                          & 7
                        &                    & 0                 &     & 317 & (5) %&
                        %79.25
                        & 1.96 % = (1.98 * 312 + 0.83 * 5)/(312+5)
												& 5.25 % = (5.31 * 504 + 3.23 * 15)/(504+15)
												\\
			\hline \tool{CoFloCo}            & 22           & 197
                        & (1)                                 & 66
                        &                                              & 5
                        &                    & 0                 &     & 290 & (1) % &
                        % 72.5
                        & 0.59 % = (0.59 * 289 + 0.71 * 1)/(289+1)
												& 2.68 % = (2.74 * 504 + 0.82 * 15)/(504+15)
												\\
			\hline \tool{KoAT1}              & 25           & 170
                        & (1)                                 & 74
                        &                                              & 12
                        &                     & 8                 & (3) & 289 & (4) %&
                        %72.25
                        & 0.96 % = (0.96 * 285 + 1.29 * 4)/(285+4)
												& 3.49 % = (3.49 * 504 + 3.37 * 15)/(504+15)
												\\
			\hline \tool{Loopus}             & 17           & 171
                        & (1)                                 & 50
                        & (1)                                          & 6
                        & (1)                 & 0                 &     & 244 & (3) %& 61
                        & 0.40 % = (0.40 * 241 + 0.56 * 3)/(241+3)
												& 0.40 % = (0.40 * 504 + 0.56 * 15)/(504+15)
												\\
		\end{tabular}
	}
	\caption{Evaluation on the Collection \tool{CINT${}^+$} \vspace*{-.4cm}}
	\label{fig:CINT}
        \vspace*{-.1cm}
\end{table}

\Cref{fig:CINT} gives the results of our evaluation, where as in \emph{TermComp}, we used a timeout of 5 minutes per example.
%
The first entry in every cell denotes the number of benchmarks from \tool{CINT${}^+$} for which the tool inferred the respective bound.
%
The number in brackets only considers the 15 new examples.
%
The runtime bounds computed by the tools are compared asymptotically as functions which depend on the largest initial absolute value $n$ of all program variables.
%
So for example, \tool{KoAT2\,\!+\,\!SIZE} proved a linear runtime bound for $231 + 2 = 233$ benchmarks, i.e., $\rc(\state)\in\landau(n)$ holds for all initial states where $|\state(v)|\leq n$ for all $v\in\VSet$.
%
Overall, this configuration succeeds on 358 examples, i.e., ``$< \omega$'' is the number
of examples where a finite bound on the runtime complexity could be computed by the tool
within the time limit.
%
%% The column ``SR'' gives the success rate on the at most 400 terminating\footnote{The tool \tool{iRankFinder} \cite{domenech2018IRankFinder} proves non-termination for 119 of 519 programs in \tool{CINT${}^+$}.} examples.
%
``$\mathrm{AVG^+(s)}$'' denotes the average runtime of successful runs in seconds, whereas ``$\mathrm{AVG(s)}$'' is the average runtime of all runs.\oldcomment{JG We should add a discussion of the experimental results and stress that KoAT2+SIZE is particularly good for examples with non-linear arithmetic (in particular those, where the improvement of \cite{lommen2022AutomaticComplexityAnalysis}
	alone is not sufficient).
	%
	We should also mention that CINT contains almost only examples with linear arithmetic and that the existing tools can already analyze almost all its examples which could be terminating.
	%
	TODO}\oldcomment{JG Should we also mention the third-party tools of KoAT (i.e., Z3, Apron, iRankFinder) and the hardware details or is it enough to do that on the website?
	%
	NL No, I don't think we shouldn't mention them here.
	%
	We don't discuss invariant or cfr in this paper.
	%
	So, we do not need to mention Apron or iRankFinder here.
	%
	Furthermore, we do not (explicitly) solve any SMT problems in this paper, too.
	%
	\\
	JG But Sympy was mentioned.
	%
	Therefore, I now also added the other third-party tools.
}

Already on the original benchmarks \tool{CINT}, integrating our novel technique for the inference of size bounds leads to the most powerful approach for runtime complexity analysis.
%
The effect of the new size bound technique becomes even clearer when also considering our new examples which contain non-linear arithmetic and loops whose runtime depends on the results of earlier loops in the program.
%
Thus, %our experiments show that
the new contributions of the paper are crucial in order to extend automated complexity analysis to larger programs with non-linear arithmetic.

\KoAT's source code, a binary, and a Docker image are available at\comment{NL I try to
  change the current url \url{https://aprove-developers.github.io/KoAT2_webpage/size} to
  this one soon.}\comment{JG I looked at the web site and I think that the following things still have
  to be done:
  \begin{itemize}
  \item Several of the links do not work yet.
  \item Why are there two links for the Docker image (one of them refers to the TWN paper)
    and the web interface?
    \item There should also be links to descriptions of the web interface, the Docker
      image, and the static binary.
      \item The text which describes the numbers in the experiments tables as well as the
        numbers in the tables do not correspond to the numbers in the paper.
      \item The tool output of KoAT2 cannot be downloaded.
        \item The examples cannot be downloaded.
      \item The table for Complexity ITS Non\_Linear is empty.
        \item Maybe the new example collections should not be called ``\ldots
          Non\_Linear'', because we already used that name in the IJCAR paper. Probably we
          should rather call them ``\ldots Size\_Non\_Linear''.
          \item In the description of the examples, I replaced ``bounded polynomial
            variables'' by ``variables with polynomial size bounds'', ok?
            \end{itemize}
  }
\url{https://koat.verify.rwth-aachen.de/size}.
%
This website also has details on our experiments, a list and description of the new
examples, and \emph{web interfaces} to run \KoAT's configurations directly online.

